Decoding Matters: Addressing Amplification Bias and Homogeneity Issue for LLM-based Recommendation

Adapting Large Language Models (LLMs) for recommendation requires careful consideration of the decoding process, given the inherent differences between generating items and natural language. Existing approaches often directly apply LLMs' original decoding methods. However, we find these methods encounter significant challenges: 1) amplification bias -- where standard length normalization inflates scores for items containing tokens with generation probabilities close to 1 (termed ghost tokens), and 2) homogeneity issue -- generating multiple similar or repetitive items for a user. To tackle these challenges, we introduce a new decoding approach named Debiasing-Diversifying Decoding (D3). D3 disables length normalization for ghost tokens to alleviate amplification bias, and it incorporates a text-free assistant model to encourage tokens less frequently generated by LLMs for counteracting recommendation homogeneity. Extensive experiments on real-world datasets demonstrate the method's effectiveness in enhancing accuracy and diversity. The code is available at https://github.com/SAI990323/DecodingMatters.

==> latex/table/table_case_study.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{p{15cm}}
    \toprule
        \multicolumn{1}{c}{\textit{Toys}} \\ \hdashline 
    \textbf{History Interaction:}  \\ \hdashline
    \textbf{Origin Recommendations:}
    \\ \hdashline
    \textbf{Refine Recommendations:}
   
\midrule
        \multicolumn{1}{c}{\textit{Sports}} \\ \hdashline 
    \textbf{History Interaction:}  \\ \hdashline
    \textbf{Origin Recommendations:}
\\ \hdashline
    \textbf{Refine Recommendations:} \\
\midrule
\multicolumn{1}{c}{\textit{Books}} \\ \hdashline 
\textbf{History Interaction:} 
\\ \hdashline
\textbf{Original Recommendations:} 
 \\ \hdashline
\textbf{Refine Recommendations:} 




% "Yamaha PKBB1 Adjustable Padded Keyboard X-Style Bench, black"
% "Yamaha EZ220 Keyboard with Lighted Keys - Includes X-Style Stand and Power Adapter"
% "M-Audio SP-2 | Universal Sustain Pedal with Piano Style Action for Electronic Keyboards"
% "Yamaha PA130 120 Volt Keyboard AC Power Adaptor"
% "ChromaCast CC-PS-MSTAND Pro Series Folding Music Stand" **
    % \hdashline
    
    \bottomrule
    \end{tabular}
    \caption{This table }
    \label{tab:case_study}
\end{table*}

\begin{table*}[]
    \centering
    \begin{tabular}{p{15cm}}
    \toprule
        \multicolumn{1}{c}{\textit{Instruments}} \\ \hdashline 
    \textbf{History Interaction:} ``Vic Firth Drumstick, (7A)'', ``Yamaha FC5 Compact Sustain Pedal for Portable Keyboards, black'' \\ \hdashline
    \textbf{Origin Recommendations:}
    ``Yamaha PKBB1 Adjustable Padded Keyboard X-Style Bench, black'',
``Yamaha EZ220 Keyboard with Lighted Keys - Includes X-Style Stand and Power Adapter'',
``Yamaha LP7A 3-Pedal Unit for DGX-660, Black'',
``Yamaha PA130 120 Volt Keyboard AC Power Adaptor'',
``Yamaha PSRE243 61-Key Portable Keyboard'' \\ \hdashline
    \textbf{Refine Recommendations:}
    ``Yamaha PKBB1 Adjustable Padded Keyboard X-Style Bench, black'',
``Yamaha EZ220 Keyboard with Lighted Keys - Includes X-Style Stand and Power Adapter'',
``M-Audio SP-2 | Universal Sustain Pedal with Piano Style Action for Electronic Keyboards'',
``Yamaha PA130 120 Volt Keyboard AC Power Adaptor'',
``\textcolor{red}{\textbf{ChromaCast CC-PS-MSTAND Pro Series Folding Music Stand}}''
\midrule
        \multicolumn{1}{c}{\textit{CDs}} \\ \hdashline 
    \textbf{History Interaction:} ``The Best Of Gerald Levert'', ``The Best Of Deniece Williams: Gonna Take A Miracle'', ``George Duke - Greatest Hits'', ``Herb Alpert \& The Tijuana Brass Greatest Hits'', ``The Best of George Benson'', ``Dance of Life'' \\ \hdashline
    \textbf{Origin Recommendations:}
``Millennium Collection - 20th Century Masters'',
``Millennium Collection - 20th Century Masters Jewel'',
``Millennium Collection - 20th Century Masters, Vol. 2'',
``Millennium Collection - 20th Century Masters - Cameo'',
``The Best of Anita Baker''
\\ \hdashline
    \textbf{Refine Recommendations:}
    ``Millennium Collection - 20th Century Masters'',
``\textcolor{red}{\textbf{Babyface - A Collection of His Greatest Hits}}'', 
``The Best Of Loose Ends -  Loose Ends'',
``Millennium Collection - 20th Century Masters Jewel  Jewel'',
``The Essential Harold Melvin \& the Blue Notes'' \\
\midrule
\multicolumn{1}{c}{\textit{Games}} \\ \hdashline 
\textbf{History Interaction:} 
``Ghostbusters - Nintendo DS'', ``Speed Racer: The Videogame - Nintendo DS'', ``Ghostbusters - Nintendo DS'', ``Speed Racer: The Videogame - Nintendo DS'', ``Pokemon Ranger: Shadows of Almia'', ``Scooby Doo! First Frights NDS'', ``Sonic All Star Racing - Nintendo DS'', ``Mario Kart 7'', ``Ben 10 Protector of Earth', 'Ben 10 Galactic Racing - Nintendo 3DS'' \\ \hdashline
\textbf{Original Recommendations:} 
``Rocksmith 2014 Edition - Xbox 360 (Cable Included)",
``Rocksmith 2014 Edition - "No Cable Included" Version for Rocksmith Owners - Playstation 3'',
``Rocksmith 2014 Edition - Playstation 3 (Cable Included)'',
``Rocksmith Real Tone USB Audio Cable [Ubisoft]'',
``Rocksmith 2014 Edition - PlayStation 4'' \\ \hdashline
\textbf{Refine Recommendations:} 
``Rocksmith 2014 Edition - Xbox 360 (Cable Included)''
``Nintendo Wii U Deluxe Set: Super Mario 3D World and Nintendo Land Bundle - Black 32 GB''
``Nintendo Wii U Deluxe Set: Super Mario Bros U \& Luigi U (32 GB)''
``Just Dance 2014 - Nintendo Wii U''
``\textcolor{red}{\textbf{Just Dance 2015 - Wii U}}''



% "Yamaha PKBB1 Adjustable Padded Keyboard X-Style Bench, black"
% "Yamaha EZ220 Keyboard with Lighted Keys - Includes X-Style Stand and Power Adapter"
% "M-Audio SP-2 | Universal Sustain Pedal with Piano Style Action for Electronic Keyboards"
% "Yamaha PA130 120 Volt Keyboard AC Power Adaptor"
% "ChromaCast CC-PS-MSTAND Pro Series Folding Music Stand" **
    % \hdashline
    
    \bottomrule
    \end{tabular}
    \caption{This table }
    \label{tab:case_study}
\end{table*}
